Learning to Generate Code Comments from Class Hierarchies

Descriptive code comments are essential for supporting code comprehension and maintenance. We propose the task of automatically generating comments for overriding methods. We formulate a novel framework which accommodates the unique contextual and linguistic reasoning that is required for performing this task. Our approach features: (1) incorporating context from the class hierarchy; (2) conditioning on learned, latent representations of specificity to generate comments that capture the more specialized behavior of the overriding method; and (3) unlikelihood training to discourage predictions which do not conform to invariant characteristics of the comment corresponding to the overridden method. Our experiments show that the proposed approach is able to generate comments for overriding methods of higher quality compared to prevailing comment generation techniques.

==> tables/dataset-numbers.tex <==
% Statistics numbers of the data set
% Original parsed data set
\DefMacro{total-projects}{9745}
\DefMacro{total-hie-pairs}{51806}
\DefMacro{total-sib-pairs}{108305}

% After filter pairs (non English, no comments, no hierarchy pairs)
\DefMacro{filtered-projects}{711}
\DefMacro{filtered-hie-pairs}{29101}
\DefMacro{filtered-sib-pairs}{70394}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Comments similarity distribution among abstract and non abstract pairs.
% abstract and non-abstract methods
\DefMacro{abstract-pairs}{20455}
\DefMacro{non-abstract-pairs}{8665}

% pct of same pairs
\DefMacro{hie-total-pct}{51.0}
\DefMacro{abstract-hie-pct}{53.5}
\DefMacro{non-abstract-hie-pct}{45.3}
% Here I only measure the similarity between the different comments
% average bleu score between comments
\DefMacro{bleu-hie-pairs}{28.118}
\DefMacro{bleu-abstract-hie-pairs}{26.119}
\DefMacro{bleu-non-abstract-hie-pairs}{32.124}

% average edit distance of pairs
\DefMacro{edit-hie-pairs}{45.267}
\DefMacro{edit-abstract-hie-pairs}{43.406}
\DefMacro{edit-non-abstract-hie-pairs}{48.998}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% average number of subtokens in comments

% number of tokens of first sentence of comments in hierarchy pairs
\DefMacro{hie-sup}{12.4}
\DefMacro{hie-sub}{11.8}
\DefMacro{hie-overall}{12.1}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Dataset split and statistics for cross-projects experiments

% training set
\DefMacro{train-pairs}{26206}
\DefMacro{train-projects}{625}
\DefMacro{train-clean-diff}{11405}

% validation set
\DefMacro{valid-pairs}{1361}
\DefMacro{valid-projects}{58}
\DefMacro{valid-clean-diff}{567}

% test set
\DefMacro{test-pairs}{1534}
\DefMacro{test-projects}{28}
\DefMacro{test-clean-diff}{614}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Performance of different models.
% If use mix dataset, with suffix mix.

% Train only on different pairs, and disjoint dataset
\DefMacro{diff-CopyGen-BLEU}{30.608}
\DefMacro{diff-CopyGen-METEOR}{33.114}
\DefMacro{diff-CopyGen-SARI}{34.005}

% Use edit sequence model, not using any features
\DefMacro{Edit-BLEU}{16.759}
\DefMacro{Edit-METEOR}{13.343}
\DefMacro{Edit-SARI}{30.624}


\DefMacro{diff-Gen-BLEU}{6.529}
\DefMacro{diff-Gen-METEOR}{4.751}

% Copy the super comment to sub comment
\DefMacro{diff-Copy-BLEU}{24.511}
\DefMacro{diff-Copy-METEOR}{28.058}

% CopyGen + SrouceIdentifier
\DefMacro{diff-ab-code-BLEU}{24.870}
\DefMacro{diff-ab-code-METEOR}{29.394}
\DefMacro{diff-ab-code-SARI}{25.202}
% Our best model by now
\DefMacro{diff-Ours-BLEU}{25.859}
\DefMacro{diff-Ours-METEOR}{29.986}
\DefMacro{diff-Ours-SARI}{24.567}

% Train and test on all the pairs, and disjoint dataset
\DefMacro{all-Copy-BLEU}{67.800}
\DefMacro{all-Copy-METEOR}{69.556}
\DefMacro{all-CopyGen-BLEU}{60.546}
\DefMacro{all-CopyGen-METEOR}{61.514}


% Old results.
%\DefMacro{diff-Copy-BLEU}{27.511}
%\DefMacro{diff-Copy-METEOR}{31.058}

\DefMacro{diff-CopyGen*-BLEU}{26.067}
\DefMacro{diff-CopyGen*-METEOR}{30.299}
\DefMacro{diff-CopyGen*-SARI}{23.057}


==> tables/dataset.tex <==
\begin{table*}[ht]
\centering
\caption{Statistics for the dataset}
\label{tab:table2}
\begin{tabular}{c|l|l|c|l|l}
\hline
\textbf{\# total projects} & \textbf{\# hp} & \textbf{\# sibp} & \textbf{\# filterd projects} & \textbf{\# hp} & \textbf{\# sibp} \\
\hline
 \hline
\UseMacro{total-projects} & \UseMacro{total-hie-pairs}  & \UseMacro{total-sib-pairs}  & \UseMacro{filtered-projects} & \UseMacro{filtered-hie-pairs} & \UseMacro{filtered-sib-pairs} \\
\hline
\end{tabular}
\end{table*}


==> tables/distribution/classNum.tex <==
\begin{table*}[ht]
\centering
\caption{Distribution of class number over projects }
\label{tab:table2}
\begin{tabular}{l|c|c|c}
\hline
\textbf{Average} & \textbf{Max} & \textbf{Min} & \textbf{Median}  \\
\hline
\hline
294.8 & 13242 & 1 & 75 \\
\hline
\end{tabular}
\end{table*}


==> tables/distribution/hpairs.tex <==
\begin{table*}[ht]
\centering
\caption{Distribution of hie pairs number over projects}
\label{tab:table2}
\begin{tabular}{l|c|c|c}
\hline
\textbf{Average} & \textbf{Max} & \textbf{Min} & \textbf{Median}  \\
\hline
\hline
294.8 & 13242 & 1 & 75 \\
\hline
\end{tabular}
\end{table*}


==> tables/distribution/hpairs_comm.tex <==
\begin{table*}[ht]
\centering
\caption{Distribution of hie pairs with comments over projects}
\label{tab:table2}
\begin{tabular}{l|c|c|c}
\hline
\textbf{Average} & \textbf{Max} & \textbf{Min} & \textbf{Median}  \\
\hline
\hline
50.3 & 6263 & 1 & 5 \\
\hline
\end{tabular}
\end{table*}


==> tables/distribution/hpairs_diff_comm.tex <==
\begin{table*}[ht]
\centering
\caption{Distribution of hpairs with different comments over projects}
\label{tab:table2}
\begin{tabular}{l|c|c|c}
\hline
\textbf{Average} & \textbf{Max} & \textbf{Min} & \textbf{Median}  \\
\hline
\hline
40 & 5593 & 1 & 4 \\
\hline
\end{tabular}
\end{table*}


==> tables/distribution/hpairs_nonab_diff.tex <==
\begin{table*}[ht]
\centering
\caption{Distribution of nonabstract hpairs with different comments over projects}
\label{tab:table2}
\begin{tabular}{l|c|c|c}
\hline
\textbf{Average} & \textbf{Max} & \textbf{Min} & \textbf{Median}  \\
\hline
\hline
10 & 2389 & 0 & 0 \\
\hline
\end{tabular}
\end{table*}


==> tables/distribution/loc.tex <==
\begin{table*}[ht]
\centering
\caption{Distribution of lines of code over projects}
\label{tab:table2}
\begin{tabular}{l|c|c|c}
\hline
\textbf{Average} & \textbf{Max} & \textbf{Min} & \textbf{Median}  \\
\hline
\hline
51235 & 1293568 & 163 & 13596 \\
\hline
\end{tabular}
\end{table*}


==> tables/distribution/methodNum.tex <==
\begin{table*}[ht]
\centering
\caption{Distribution of method number over projects}
\label{tab:table2}
\begin{tabular}{l|c|c|c}
\hline
\textbf{Average} & \textbf{Max} & \textbf{Min} & \textbf{Median}  \\
\hline
\hline
1014.9 & 44539 & 2 & 274 \\
\hline
\end{tabular}
\end{table*}


==> tables/distribution/spairs_comm.tex <==
\begin{table*}[ht]
\centering
\caption{Distribution of spairs with comments over projects}
\label{tab:table2}
\begin{tabular}{l|c|c|c}
\hline
\textbf{Average} & \textbf{Max} & \textbf{Min} & \textbf{Median}  \\
\hline
\hline
151 & 30004 & 0 & 0\\
\hline
\end{tabular}
\end{table*}


==> tables/distribution/spairs_diff_comm.tex <==
\begin{table*}[ht]
\centering
\caption{Distribution of spairs with different comments over projects}
\label{tab:table2}
\begin{tabular}{l|c|c|c}
\hline
\textbf{Average} & \textbf{Max} & \textbf{Min} & \textbf{Median}  \\
\hline
\hline
84 & 20387 & 0 & 0 \\
\hline
\end{tabular}
\end{table*}


==> tables/numbers-models-metrics.tex <==
%% Automatically generated by pyutil.latex

\DefMacro{CopyGen-short-acc}{0.187}
\DefMacro{CopyGen-short-bleu}{34.433}
\DefMacro{CopyGen-short-meteor}{29.887}
\DefMacro{CopyGen-short-sari}{35.052}
\DefMacro{CopyGen-short-gleu}{21.342}
\DefMacro{CopyGen-short-rouge-l}{52.526}
\DefMacro{CopyGen-long-acc}{0.578}
\DefMacro{CopyGen-long-bleu}{24.635}
\DefMacro{CopyGen-long-meteor}{23.478}
\DefMacro{CopyGen-long-sari}{33.356}
\DefMacro{CopyGen-long-gleu}{19.575}
\DefMacro{CopyGen-long-rouge-l}{46.684}
\DefMacro{GenModel-short-acc}{0.620}
\DefMacro{GenModel-short-bleu}{15.451}
\DefMacro{GenModel-short-meteor}{13.125}
\DefMacro{GenModel-short-sari}{35.035}
\DefMacro{GenModel-short-gleu}{15.763}
\DefMacro{GenModel-short-rouge-l}{29.453}
\DefMacro{GenModel-long-acc}{0.000}
\DefMacro{GenModel-long-bleu}{10.425}
\DefMacro{GenModel-long-meteor}{11.578}
\DefMacro{GenModel-long-sari}{33.676}
\DefMacro{GenModel-long-gleu}{10.034}
\DefMacro{GenModel-long-rouge-l}{28.165}
\DefMacro{EditModel-short-acc}{2.284}
\DefMacro{EditModel-short-bleu}{31.666}
\DefMacro{EditModel-short-meteor}{27.761}
\DefMacro{EditModel-short-sari}{38.536}
\DefMacro{EditModel-short-gleu}{20.039}
\DefMacro{EditModel-short-rouge-l}{50.010}
\DefMacro{EditModel-long-acc}{1.308}
\DefMacro{EditModel-long-bleu}{22.232}
\DefMacro{EditModel-long-meteor}{21.729}
\DefMacro{EditModel-long-sari}{37.479}
\DefMacro{EditModel-long-gleu}{14.316}
\DefMacro{EditModel-long-rouge-l}{45.186}
\DefMacro{EditGen-short-acc}{4.608}
\DefMacro{EditGen-short-bleu}{35.531}
\DefMacro{EditGen-short-meteor}{29.971}
\DefMacro{EditGen-short-sari}{31.397}
\DefMacro{EditGen-short-gleu}{24.659}
\DefMacro{EditGen-short-rouge-l}{51.001}
\DefMacro{EditGen-long-acc}{3.083}
\DefMacro{EditGen-long-bleu}{24.667}
\DefMacro{EditGen-long-meteor}{23.187}
\DefMacro{EditGen-long-sari}{31.993}
\DefMacro{EditGen-long-gleu}{16.994}
\DefMacro{EditGen-long-rouge-l}{44.359}
\DefMacro{Copy-short-acc}{0.000}
\DefMacro{Copy-short-bleu}{24.228}
\DefMacro{Copy-short-meteor}{19.845}
\DefMacro{Copy-short-sari}{14.135}
\DefMacro{Copy-short-gleu}{18.988}
\DefMacro{Copy-short-rouge-l}{43.352}
\DefMacro{Copy-long-acc}{0.000}
\DefMacro{Copy-long-bleu}{20.623}
\DefMacro{Copy-long-meteor}{18.757}
\DefMacro{Copy-long-sari}{14.172}
\DefMacro{Copy-long-gleu}{16.090}
\DefMacro{Copy-long-rouge-l}{40.846}
\DefMacro{ClsSubt-short-acc}{2.672}
\DefMacro{ClsSubt-short-bleu}{26.764}
\DefMacro{ClsSubt-short-meteor}{22.496}
\DefMacro{ClsSubt-short-sari}{16.675}
\DefMacro{ClsSubt-short-gleu}{19.074}
\DefMacro{ClsSubt-short-rouge-l}{45.632}
\DefMacro{ClsSubt-long-acc}{2.312}
\DefMacro{ClsSubt-long-bleu}{24.215}
\DefMacro{ClsSubt-long-meteor}{21.442}
\DefMacro{ClsSubt-long-sari}{16.781}
\DefMacro{ClsSubt-long-gleu}{16.388}
\DefMacro{ClsSubt-long-rouge-l}{42.014}
\DefMacro{BestEnsemble-short-acc}{6.048}
\DefMacro{BestEnsemble-short-bleu}{41.420}
\DefMacro{BestEnsemble-short-meteor}{35.398}
\DefMacro{BestEnsemble-short-sari}{41.864}
\DefMacro{BestEnsemble-short-gleu}{29.518}
\DefMacro{BestEnsemble-short-rouge-l}{57.534}
\DefMacro{BestEnsemble-long-acc}{4.753}
\DefMacro{BestEnsemble-long-bleu}{34.764}
\DefMacro{BestEnsemble-long-meteor}{31.783}
\DefMacro{BestEnsemble-long-sari}{37.036}
\DefMacro{BestEnsemble-long-gleu}{23.032}
\DefMacro{BestEnsemble-long-rouge-l}{53.610}

\DefMacro{Ensemble-short-acc}{2.544}
\DefMacro{Ensemble-short-bleu}{36.448}
\DefMacro{Ensemble-short-meteor}{31.666}
\DefMacro{Ensemble-short-sari}{39.183}
\DefMacro{Ensemble-short-gleu}{28.441}
\DefMacro{Ensemble-short-rouge-l}{54.442}
\DefMacro{Ensemble-long-acc}{1.789}
\DefMacro{Ensemble-long-bleu}{25.661}
\DefMacro{Ensemble-long-meteor}{25.004}
\DefMacro{Ensemble-long-sari}{32.085}
\DefMacro{Ensemble-long-gleu}{20.031}
\DefMacro{Ensemble-long-rouge-l}{48.211}


%% Manually generated (will be implemented automatically generated later)
\DefMacro{EditGen-short-classifier}{78.3}
\DefMacro{EditGen-long-classifier}{72.1}

\DefMacro{Copy-rank-short-bleu}{24}
\DefMacro{ClsSubt-rank-short-bleu}{90}
\DefMacro{CopyGen-rank-short-bleu}{207}
\DefMacro{EditModel-rank-short-bleu}{40}
\DefMacro{GenModel-rank-short-bleu}{102}

\DefMacro{Copy-rank-short-meteor}{26}
\DefMacro{ClsSubt-rank-short-meteor}{112}
\DefMacro{CopyGen-rank-short-meteor}{206}
\DefMacro{EditModel-rank-short-meteor}{36}
\DefMacro{GenModel-rank-short-meteor}{83}

\DefMacro{Copy-rank-short-rouge}{18}
\DefMacro{ClsSubt-rank-short-rouge}{98}
\DefMacro{CopyGen-rank-short-rouge}{240}
\DefMacro{EditModel-rank-short-rouge}{41}
\DefMacro{GenModel-rank-short-rouge}{66}


\DefMacro{Copy-rank-long-bleu}{63}
\DefMacro{ClsSubt-rank-long-bleu}{105}
\DefMacro{CopyGen-rank-long-bleu}{212}
\DefMacro{EditModel-rank-long-bleu}{34}
\DefMacro{GenModel-rank-long-bleu}{105}

\DefMacro{Copy-rank-long-meteor}{69}
\DefMacro{ClsSubt-rank-long-meteor}{144}
\DefMacro{CopyGen-rank-long-meteor}{191}
\DefMacro{EditModel-rank-long-meteor}{34}
\DefMacro{GenModel-rank-long-meteor}{81}

\DefMacro{Copy-rank-long-rouge}{45}
\DefMacro{ClsSubt-rank-long-rouge}{99}
\DefMacro{CopyGen-rank-long-rouge}{257}
\DefMacro{EditModel-rank-long-rouge}{33}
\DefMacro{GenModel-rank-long-rouge}{85}

\DefMacro{AST-CopyGen-short-acc}{0.072}
\DefMacro{AST-CopyGen-short-bleu}{34.842}
\DefMacro{AST-CopyGen-short-meteor}{30.200}
\DefMacro{AST-CopyGen-short-sari}{33.272}
\DefMacro{AST-CopyGen-short-gleu}{23.674}
\DefMacro{AST-CopyGen-short-rouge-l}{52.768}
\DefMacro{AST-CopyGen-long-acc}{0.000}
\DefMacro{AST-CopyGen-long-bleu}{24.791}
\DefMacro{AST-CopyGen-long-meteor}{24.031}
\DefMacro{AST-CopyGen-long-sari}{33.087}
\DefMacro{AST-CopyGen-long-gleu}{15.480}
\DefMacro{AST-CopyGen-long-rouge-l}{47.146}

\DefMacro{DeepCom-short-acc}{0.000}
\DefMacro{DeepCom-short-bleu}{26.073}
\DefMacro{DeepCom-short-meteor}{22.256}
\DefMacro{DeepCom-short-sari}{33.213}
\DefMacro{DeepCom-short-gleu}{23.331}
\DefMacro{DeepCom-short-rouge-l}{45.037}
\DefMacro{DeepCom-long-acc}{0.000}
\DefMacro{DeepCom-long-bleu}{21.812}
\DefMacro{DeepCom-long-meteor}{20.779}
\DefMacro{DeepCom-long-sari}{33.332}
\DefMacro{DeepCom-long-gleu}{16.740}
\DefMacro{DeepCom-long-rouge-l}{40.257}

\DefMacro{CopyGen-feat-short-acc}{0.000}
\DefMacro{CopyGen-feat-short-bleu}{33.715}
\DefMacro{CopyGen-feat-short-meteor}{29.029}
\DefMacro{CopyGen-feat-short-sari}{32.929}
\DefMacro{CopyGen-feat-short-gleu}{20.736}
\DefMacro{CopyGen-feat-short-rouge-l}{52.688}
\DefMacro{CopyGen-feat-long-acc}{0.000}
\DefMacro{CopyGen-feat-long-bleu}{24.303}
\DefMacro{CopyGen-feat-long-meteor}{23.486}
\DefMacro{CopyGen-feat-long-sari}{32.921}
\DefMacro{CopyGen-feat-long-gleu}{14.424}
\DefMacro{CopyGen-feat-long-rouge-l}{46.722}
\DefMacro{CopyGen-class-short-acc}{0.000}
\DefMacro{CopyGen-class-short-bleu}{33.969}
\DefMacro{CopyGen-class-short-meteor}{28.984}
\DefMacro{CopyGen-class-short-sari}{33.114}
\DefMacro{CopyGen-class-short-gleu}{19.971}
\DefMacro{CopyGen-class-short-rouge-l}{52.098}
\DefMacro{CopyGen-class-long-acc}{0.000}
\DefMacro{CopyGen-class-long-bleu}{23.745}
\DefMacro{CopyGen-class-long-meteor}{22.887}
\DefMacro{CopyGen-class-long-sari}{33.235}
\DefMacro{CopyGen-class-long-gleu}{15.309}
\DefMacro{CopyGen-class-long-rouge-l}{46.335}
\DefMacro{CopyGen-com-short-acc}{0.000}
\DefMacro{CopyGen-com-short-bleu}{22.694}
\DefMacro{CopyGen-com-short-meteor}{21.209}
\DefMacro{CopyGen-com-short-sari}{33.764}
\DefMacro{CopyGen-com-short-gleu}{18.094}
\DefMacro{CopyGen-com-short-rouge-l}{41.948}
\DefMacro{CopyGen-com-long-acc}{0.000}
\DefMacro{CopyGen-com-long-bleu}{13.890}
\DefMacro{CopyGen-com-long-meteor}{15.115}
\DefMacro{CopyGen-com-long-sari}{33.964}
\DefMacro{CopyGen-com-long-gleu}{12.128}
\DefMacro{CopyGen-com-long-rouge-l}{33.907}

\DefMacro{meta-classifier-short-acc}{41.2}
\DefMacro{meta-classifier-long-acc}{34.6}


==> tables/projects-numbers.tex <==
% Pairs: super class and sub class's method pairs
% Both: both super and sub class's method having comments
% Niether: niether super and sub class's method having comments
% Super: only super class's method having comments
% Sub: only sub class's method having comments
% NA: both super and sub class's methods are non abstract
% Sibling: number of method sibling pairs

% google-auto project number
\DefMacro{google-autoLOC}{28189}
\DefMacro{google-auto-Classes}{766}
\DefMacro{google-auto-Methods}{2483}
\DefMacro{google-auto-Pairs}{95}
\DefMacro{google-auto-Both}{0}
\DefMacro{google-auto-Niether}{49}
\DefMacro{google-auto-Super}{45}
\DefMacro{google-auto-Sub}{1}
\DefMacro{google-auto-NA}{29}
\DefMacro{google-auto-Sibling}{44}
% collections project number
\DefMacro{collectionsLOC}{64465}
\DefMacro{collections-Classes}{758}
\DefMacro{collections-Methods}{6451}
\DefMacro{collections-Pairs}{668}
\DefMacro{collections-Both}{221}
\DefMacro{collections-Niether}{145}
\DefMacro{collections-Super}{259}
\DefMacro{collections-Sub}{43}
\DefMacro{collections-NA}{342}
\DefMacro{collections-Sibling}{476}
% dynjs project number
\DefMacro{dynjsLOC}{42431}
\DefMacro{dynjs-Classes}{741}
\DefMacro{dynjs-Methods}{4202}
\DefMacro{dynjs-Pairs}{709}
\DefMacro{dynjs-Both}{0}
\DefMacro{dynjs-Niether}{703}
\DefMacro{dynjs-Super}{6}
\DefMacro{dynjs-Sub}{0}
\DefMacro{dynjs-NA}{182}
\DefMacro{dynjs-Sibling}{1104}
% graphhopper project number
\DefMacro{graphhopperLOC}{80401}
\DefMacro{graphhopper-Classes}{921}
\DefMacro{graphhopper-Methods}{6160}
\DefMacro{graphhopper-Pairs}{871}
\DefMacro{graphhopper-Both}{17}
\DefMacro{graphhopper-Niether}{464}
\DefMacro{graphhopper-Super}{376}
\DefMacro{graphhopper-Sub}{14}
\DefMacro{graphhopper-NA}{191}
\DefMacro{graphhopper-Sibling}{319}
% guava project number
\DefMacro{guavaLOC}{395418}
\DefMacro{guava-Classes}{3552}
\DefMacro{guava-Methods}{30771}
\DefMacro{guava-Pairs}{3257}
\DefMacro{guava-Both}{315}
\DefMacro{guava-Niether}{1536}
\DefMacro{guava-Super}{1339}
\DefMacro{guava-Sub}{67}
\DefMacro{guava-NA}{1382}
\DefMacro{guava-Sibling}{1992}
% jenkins project number
\DefMacro{jenkinsLOC}{161811}
\DefMacro{jenkins-Classes}{2955}
\DefMacro{jenkins-Methods}{13935}
\DefMacro{jenkins-Pairs}{1730}
\DefMacro{jenkins-Both}{116}
\DefMacro{jenkins-Niether}{299}
\DefMacro{jenkins-Super}{1289}
\DefMacro{jenkins-Sub}{26}
\DefMacro{jenkins-NA}{694}
\DefMacro{jenkins-Sibling}{2896}
% jOQQ project number
\DefMacro{jOQQLOC}{190913}
\DefMacro{jOQQ-Classes}{1819}
\DefMacro{jOQQ-Methods}{30447}
\DefMacro{jOQQ-Pairs}{6399}
\DefMacro{jOQQ-Both}{792}
\DefMacro{jOQQ-Niether}{855}
\DefMacro{jOQQ-Super}{4598}
\DefMacro{jOQQ-Sub}{154}
\DefMacro{jOQQ-NA}{917}
\DefMacro{jOQQ-Sibling}{6792}
% stubby4j project number
\DefMacro{stubby4jLOC}{14439}
\DefMacro{stubby4j-Classes}{100}
\DefMacro{stubby4j-Methods}{1079}
\DefMacro{stubby4j-Pairs}{15}
\DefMacro{stubby4j-Both}{0}
\DefMacro{stubby4j-Niether}{15}
\DefMacro{stubby4j-Super}{0}
\DefMacro{stubby4j-Sub}{0}
\DefMacro{stubby4j-NA}{0}
\DefMacro{stubby4j-Sibling}{0}
% google-truth project number
\DefMacro{google-truthLOC}{34528}
\DefMacro{google-truth-Classes}{297}
\DefMacro{google-truth-Methods}{3632}
\DefMacro{google-truth-Pairs}{250}
\DefMacro{google-truth-Both}{6}
\DefMacro{google-truth-Niether}{27}
\DefMacro{google-truth-Super}{214}
\DefMacro{google-truth-Sub}{3}
\DefMacro{google-truth-NA}{36}
\DefMacro{google-truth-Sibling}{31}

% vraptor4 project number
\DefMacro{vraptor4LOC}{27496}
\DefMacro{vraptor4-Classes}{699}
\DefMacro{vraptor4-Methods}{2827}
\DefMacro{vraptor4-Pairs}{348}
\DefMacro{vraptor4-Both}{6}
\DefMacro{vraptor4-Niether}{173}
\DefMacro{vraptor4-Super}{168}
\DefMacro{vraptor4-Sub}{1}
\DefMacro{vraptor4-NA}{10}
\DefMacro{vraptor4-Sibling}{52}


==> tables/projects.tex <==
\begin{table*}[ht]
\centering
\caption{hierarchy results got by parsing 10 github projects}
\label{tab:table5}
\begin{tabular}{l|c|c|c}
\hline
\textbf{Project} & \textbf{LOC} & \textbf{\#Classes} & \textbf{\#Methods} \\
\hline
\hline
\UseMacro{google-auto} & \UseMacro{google-autoLOC} & \UseMacro{google-auto-Classes} & \UseMacro{google-auto-Methods} \\
\hline
\UseMacro{collections} & \UseMacro{collectionsLOC} & \UseMacro{collections-Classes} & \UseMacro{collections-Methods} \\
\hline
\UseMacro{dynjs} & \UseMacro{dynjsLOC} & \UseMacro{dynjs-Classes} & \UseMacro{dynjs-Methods} \\
\hline
\UseMacro{graphhopper} & \UseMacro{graphhopperLOC} & \UseMacro{graphhopper-Classes} & \UseMacro{graphhopper-Methods} \\
\hline
\UseMacro{guava} & \UseMacro{guavaLOC} & \UseMacro{guava-Classes} & \UseMacro{guava-Methods} \\
\hline
\UseMacro{jenkins} & \UseMacro{jenkinsLOC} & \UseMacro{jenkins-Classes} & \UseMacro{jenkins-Methods} \\
\hline
\UseMacro{jOQQ} & \UseMacro{jOQQLOC} & \UseMacro{jOQQ-Classes} & \UseMacro{jOQQ-Methods} \\
\hline
\UseMacro{stubby4j} & \UseMacro{stubby4jLOC} & \UseMacro{stubby4j-Classes} & \UseMacro{stubby4j-Methods} \\
\hline
\UseMacro{google-truth} & \UseMacro{google-truthLOC} & \UseMacro{google-truth-Classes} & \UseMacro{google-truth-Methods} \\
\hline
\UseMacro{vraptor4} & \UseMacro{vraptor4LOC} & \UseMacro{vraptor4-Classes} & \UseMacro{vraptor4-Methods} \\
\hline
\end{tabular}
\end{table*}


==> tables/table-ab-bleu.tex <==
\begin{table*}[ht]
\centering
\caption{Models performance on abstract methods.}
\label{tab:table6}
\begin{tabular}{c|c|c}
\hline
\textbf{} & \textbf{Abstract} & \textbf{NonAbstract}  \\
\hline
\hline
Copy & 23.05 & 20.47 \\
ClassSubt & 22.47 & 20.56 \\
CopyGen & 23.39 & 21.40 \\ 
\hline
\end{tabular}
\end{table*}


==> tables/table-ab-comlen.tex <==
\begin{table*}[ht]
\centering
\caption{Average number of sub-tokens of ab/comments}
\label{tab:comm-len}
\begin{tabular}{l|c|c|c|c}
\hline
\textbf{Pairs} & \textbf{abstract sup} & \textbf{abstract sub} & \textbf{nonab sup} & \textbf{nonab sub}\\
\hline
\hline
first sentence comments & \UseMacro{short-abstract-sup-comments-tokens} & \UseMacro{short-abstract-sub-comments-tokens} & \UseMacro{short-nonabstract-sup-comments-tokens} & \UseMacro{short-nonabstract-sub-comments-tokens}  \\
whole comments & \UseMacro{long-abstract-sup-comments-tokens} & \UseMacro{long-abstract-sub-comments-tokens} & \UseMacro{long-nonabstract-sup-comments-tokens} & \UseMacro{long-nonabstract-sub-comments-tokens} \\
\hline
\end{tabular}
\end{table*}


==> tables/table-ablation.tex <==

%% Automatically generated by pyutil.latex 

\begin{table*}[ht]
\small
\centering
\begin{tabular}{c|cllll}
\toprule
 \textbf{Dataset} & & \textbf{Model} & \textbf{BLEU-4} & \textbf{METEOR} &\textbf{ROUGE-L} \\
\midrule
\multirow{5}{*}{\Short{}} &
(1) &
{\small\SuperAwareGenWithSpecRerank{}}
  & \textbf{\UseMacro{CopyGen-neg-remove-overlap-short-bleu}}
  & \textbf{\UseMacro{CopyGen-neg-remove-overlap-short-meteor}}
  & \textbf{\UseMacro{CopyGen-neg-remove-overlap-short-rouge-l}}
\\
&
(2) &
{\hspace{0.2cm}\small\SuperAwareGenWOutUll{}}
 & \UseMacro{CopyGen-wo-ull-short-bleu}
 & \UseMacro{CopyGen-wo-ull-short-meteor}
 & \UseMacro{CopyGen-wo-ull-short-rouge-l}
\\
&
(3) &
{\hspace{0.2cm}\small\SuperAwareGenWOutSpecWOutRerank{}}
 & \UseMacro{CopyGen-short-bleu}
 & \UseMacro{CopyGen-short-meteor}$^{\eta}$
 & \UseMacro{CopyGen-short-rouge-l}$^{\zeta}$
\\
&
(4) &
{\hspace{0.2cm}\small\SuperAwareGenWOutFeatWOutRerankWOutSpec{}}
 & \UseMacro{CopyGen-feat-short-bleu}$^{\alpha}$
 & \UseMacro{CopyGen-feat-short-meteor}
 & \UseMacro{CopyGen-feat-short-rouge-l}$^{\zeta}$
\\
&
(5) &
{\hspace{0.2cm}\small\SuperAwareGenWOutClassName{}}
 & \UseMacro{CopyGen-class-short-bleu}$^{\alpha}$
 & \UseMacro{CopyGen-class-short-meteor}$^{\eta}$
 & \UseMacro{CopyGen-class-short-rouge-l}
\\
&
(6) &
{\hspace{0.2cm}\small\SuperAwareGenWOutComment{}}
 & \UseMacro{CopyGen-com-short-bleu}
 & \UseMacro{CopyGen-com-short-meteor}
 & \UseMacro{CopyGen-com-short-rouge-l}
\\
%% &
%% {\small\SuperAgnosticModel{}}
%%  & \UseMacro{GenModel-short-bleu}
%%  & \UseMacro{GenModel-short-meteor}
%%  & \UseMacro{GenModel-short-rouge-l}
%% \\
%% &
%% {\small\SuperAwareGenWOutRerankWOutSpecWithAST{}}
%%  & \UseMacro{AST-CopyGen-short-bleu}
%%  & \UseMacro{AST-CopyGen-short-meteor}
%%  & \UseMacro{AST-CopyGen-short-rouge-l}
%% \\

%% &
\midrule
\multirow{5}{*}{\Long{}} &
(1) &
{\small\SuperAwareGenWithSpecRerank{}}
  & \textbf{\UseMacro{CopyGen-neg-remove-overlap-long-bleu}}
  & \textbf{\UseMacro{CopyGen-neg-remove-overlap-long-meteor}}
  & \textbf{\UseMacro{CopyGen-neg-remove-overlap-long-rouge-l}}$^{\psi}$
\\
&
(2) &
{\hspace{0.2cm}\small\SuperAwareGenWOutUll{}}
 & \UseMacro{CopyGen-wo-ull-long-bleu}
 & \UseMacro{CopyGen-wo-ull-long-meteor}
 & \UseMacro{CopyGen-wo-ull-long-rouge-l}$^{\psi}$
\\
&
(3) &
{\hspace{0.2cm}\small\SuperAwareGenWOutSpecWOutRerank{}}
 & \UseMacro{CopyGen-long-bleu}$^{\delta\theta}$
 & \UseMacro{CopyGen-long-meteor}$^{\epsilon}$
 & \UseMacro{CopyGen-long-rouge-l}$^{\gamma\kappa}$
\\
&
(4) &
{\hspace{0.2cm}\small\SuperAwareGenWOutFeatWOutRerankWOutSpec{}}
 & \UseMacro{CopyGen-feat-long-bleu}$^{\theta}$
 & \UseMacro{CopyGen-feat-long-meteor}$^{\epsilon}$
 & \UseMacro{CopyGen-feat-long-rouge-l}$^{\gamma}$
\\
&
(5) &
{\hspace{0.2cm}\small\SuperAwareGenWOutClassName{}}
 & \UseMacro{CopyGen-class-long-bleu}$^{\delta}$
 & \UseMacro{CopyGen-class-long-meteor}
 & \UseMacro{CopyGen-class-long-rouge-l}$^{\kappa}$
\\
&
(6) &
{\hspace{0.2cm}\small\SuperAwareGenWOutComment{}}
 & \UseMacro{CopyGen-com-long-bleu}
 & \UseMacro{CopyGen-com-long-meteor}
 & \UseMacro{CopyGen-com-long-rouge-l}
\\
%% &
%% {\small\SuperAgnosticModel{}}
%%  & \UseMacro{GenModel-long-bleu}
%%  & \UseMacro{GenModel-long-meteor}
%%  & \UseMacro{GenModel-long-rouge-l}
%% \\
%% &
%% {\small\SuperAwareGenWOutRerankWOutSpecWithAST{}}
%%  & \UseMacro{AST-CopyGen-long-bleu}
%%  & \UseMacro{AST-CopyGen-long-meteor}
%%  & \UseMacro{AST-CopyGen-long-rouge-l}
%% \\

%% &
\bottomrule
\end{tabular}
\caption{\TableCaptionAblation}
\end{table*}


==> tables/table-abstract-comlen.tex <==
\begin{table*}[ht]
\centering
\caption{Average number of tokens of whole javadoc comments}
\label{tab:comm-len}
\begin{tabular}{l|c|c|c|c}
\hline
 & \textbf{abstract sup comm} & \textbf{abstract sub comm} & \textbf{nonab sup comm} & \textbf{nonab sub comm}\\
\hline
\hline
whole comments & 27.57 & 21.72 & 36.96 & 27.91 \\
\hline
\end{tabular}
\end{table*}


==> tables/table-comlen.tex <==
\begin{table}
  \resizebox{\linewidth}{!}{
\centering

\begin{tabular}{l|c|c}
\hline
\textbf{} & \textbf{\ParentComment{}} & \textbf{\Comment{}} \\
\hline
\hline
short & \UseMacro{short-sup-comments-tokens} & \UseMacro{short-sub-comments-tokens}  \\
long & \UseMacro{long-sup-comments-tokens} & \UseMacro{long-sub-comments-tokens} \\
\hline
\end{tabular}
  }
\caption{Average number of sub-tokens of sup/sub comments}\label{tab:comm-len}
 
\end{table}


==> tables/table-editgen-result.tex <==
\begin{table*}[ht]
\centering
\caption{Model performance.}
\label{tab:short-results}
\begin{tabular}{c|c|c|c|c}
\hline
\textbf{Model} & \textbf{Accuracy} & \textbf{BLEU-4} & \textbf{METEOR} & \textbf{SARI}  \\
\hline
\hline
Classifier & 0.753 &- &-&- \\
\hline
EditGen & - & 32.952 & 28.258 & 39.563 \\
\hline
\end{tabular}
\end{table*}


==> tables/table-merged-dataset-metrics.tex <==
% Manually merged from table-dataset-metrics and table-old-dataset-metrics
% Not including #projects before preprocessing

\begin{table*}
\small
\centering
\begin{tabular}{l|rrrcc}
\toprule
\textbf{} & \textbf{Train} & \textbf{Valid} & \textbf{Test} & \textbf{Avg. len(\ParentComment{})} & \textbf{Avg. len(\ChildComment{})} \\
\midrule
\#Projects &
\UseMacro{train-projects} &
\UseMacro{valid-projects} &
\UseMacro{test-projects} &
\TableHeadNA &
\TableHeadNA \\
\midrule
Comments (before preprocessing) &
\UseMacro{raw-train-pairs} &
\UseMacro{raw-valid-pairs} &
\UseMacro{raw-test-pairs} &
\TableHeadNA &
\TableHeadNA \\
%% \#Projects&
%% \UseMacro{raw-train-projects} &
%% \UseMacro{raw-valid-projects} &
%% \UseMacro{raw-test-projects} &
%% n/a &
%% n/a \\
%\#Projects &
%\UseMacro{train-projects} &
%\UseMacro{valid-projects} &
%\UseMacro{test-projects} &
%n/a &
%n/a \\
\midrule
\Short{} &
\UseMacro{short-train-numbers} &
\UseMacro{short-valid-numbers} &
\UseMacro{short-test-numbers} &
\UseMacro{short-sup-comments-tokens} &
\UseMacro{short-sub-comments-tokens}  \\
\Long{} &
\UseMacro{long-train-numbers} &
\UseMacro{long-valid-numbers} &
\UseMacro{long-test-numbers} &
\UseMacro{long-sup-comments-tokens} &
\UseMacro{long-sub-comments-tokens} \\
\bottomrule
\end{tabular}
\caption{Number of projects; total number of comments before preprocessing (same for \xshort and \xlong); the number of examples after preprocessing (for \xshort and \xlong); and average number of subtokens in \ParentComment{} and
  \ChildComment{} in \xshort and \xlong
  datasets.\label{tab:ds-merged-metrics}}
\end{table*}


==> tables/table-meta-classifier.tex <==

%% Automatically generated by pyutil.latex 

\begin{table}
\resizebox{\linewidth}{!}{
\centering
\begin{tabular}{l|c|c}
\hline
\textbf{Model} & \textbf{} & \textbf{Accuracy} \\
\hline
\multirow{2}{*}{Meta-classifier} &
First-sentence
& \UseMacro{meta-classifier-short-acc}\\
&
Full description
& \UseMacro{meta-classifier-long-acc}\\
\hline
\end{tabular}
}
\caption{Accuracy of Meta-classifier.}\label{tab:meta-clasf}\SheenaComment{I don't think you need the left-most column.}
\end{table}


==> tables/table-models-metrics-long.tex <==

\begin{table*}
\scriptsize
  \begin{small}
\resizebox{\linewidth}{!}{
\centering
\begin{tabular}{c|ccc|ccc}
  \hline
  &
  \multicolumn{3}{c|}{\Short{}}
  &
  \multicolumn{3}{c}{\Long{}}
  \\
  \hline
\textbf{Model} & \textbf{BLEU-4} & \textbf{METEOR} &\textbf{ROUGE-l}
& \textbf{BLEU-4} & \textbf{METEOR} &\textbf{ROUGE-l}\\
\hline
\UseMacro{Copy}
 & \UseMacro{Copy-short-bleu}
 & \UseMacro{Copy-short-meteor}
 & \UseMacro{Copy-short-rouge-l}
 & \UseMacro{Copy-long-bleu}
 & \UseMacro{Copy-long-meteor}
 & \UseMacro{Copy-long-rouge-l}
\\
\UseMacro{DeepCom}
 & \UseMacro{DeepCom-short-bleu}
 & \UseMacro{DeepCom-short-meteor}
 & \UseMacro{DeepCom-short-rouge-l}
 & \UseMacro{DeepCom-long-bleu}
 & \UseMacro{DeepCom-long-meteor}
 & \UseMacro{DeepCom-long-rouge-l}
\\
\UseMacro{ClsSubt}
 & \UseMacro{ClsSubt-short-bleu}
 & \UseMacro{ClsSubt-short-meteor}
 & \UseMacro{ClsSubt-short-rouge-l}
 & \UseMacro{ClsSubt-long-bleu}
 & \UseMacro{ClsSubt-long-meteor}
 & \UseMacro{ClsSubt-long-rouge-l}
%% \\
%% \UseMacro{GenModel}
%%  & \UseMacro{GenModel-long-bleu}
%%  & \UseMacro{GenModel-long-meteor}
%%  & \UseMacro{GenModel-long-rouge-l}
\\
\UseMacro{EditModel}
 & \UseMacro{EditModel-short-bleu}
 & \UseMacro{EditModel-short-meteor}
 & \UseMacro{EditModel-short-rouge-l}
 & \UseMacro{EditModel-long-bleu}
 & \UseMacro{EditModel-long-meteor}
 & \UseMacro{EditModel-long-rouge-l}
\\
\UseMacro{CopyGen-spec-rerank}
 & \textbf{\UseMacro{CopyGen-spec-rerank-short-bleu}}
 & \textbf{\UseMacro{CopyGen-spec-rerank-short-meteor}}
 & \textbf{\UseMacro{CopyGen-spec-rerank-short-rouge-l}}
 & \textbf{\UseMacro{CopyGen-spec-rerank-long-bleu}}
 & \textbf{\UseMacro{CopyGen-spec-rerank-long-meteor}}
 & \textbf{\UseMacro{CopyGen-spec-rerank-long-rouge-l}}
\\
\hline
\end{tabular}
}
\end{small}
\caption{Comparison of our proposed approach with the baseline
  methods.}\label{tab:results}
\end{table*}


==> tables/table-models-metrics-short.tex <==

\begin{table}
\resizebox{\linewidth}{!}{
\centering
\begin{tabular}{c|ccc}
\hline
\textbf{Model} & \textbf{BLEU-4} & \textbf{METEOR} &\textbf{ROUGE-l} \\
\hline
\UseMacro{Copy}
 & \UseMacro{Copy-short-bleu}
 & \UseMacro{Copy-short-meteor}
 & \UseMacro{Copy-short-rouge-l}
\\
\UseMacro{DeepCom}
 & \UseMacro{DeepCom-short-bleu}
 & \UseMacro{DeepCom-short-meteor}
& \UseMacro{DeepCom-short-rouge-l}
\\
\UseMacro{ClsSubt}
 & \UseMacro{ClsSubt-short-bleu}
 & \UseMacro{ClsSubt-short-meteor}
 & \UseMacro{ClsSubt-short-rouge-l}
%% \\
%% \UseMacro{GenModel}
%%  & \UseMacro{GenModel-short-bleu}
%%  & \UseMacro{GenModel-short-meteor}
%%  & \UseMacro{GenModel-short-rouge-l}
\\
\UseMacro{EditModel}
 & \UseMacro{EditModel-short-bleu}
 & \UseMacro{EditModel-short-meteor}
 & \UseMacro{EditModel-short-rouge-l}
\\
\UseMacro{CopyGen-spec-rerank}
 & \textbf{\UseMacro{CopyGen-spec-rerank-short-bleu}}
 & \textbf{\UseMacro{CopyGen-spec-rerank-short-meteor}}
 & \textbf{\UseMacro{CopyGen-spec-rerank-short-rouge-l}}
\\
\hline
\end{tabular}
}
\caption{Comparison of our proposed approach with the baseline methods
  for first.}\label{tab:short-results}
\end{table}


==> tables/table-models-rank-long.tex <==

%% Automatically generated by pyutil.latex 

\begin{table*}[ht]
\centering
\caption{Models number of rank 1st in long comment generation task}
\begin{tabular}{c|c|c|c|c|c|c}
\hline
\textbf{Model} & \textbf{BLEU-4} & \textbf{METEOR} &\textbf{ROUGE-l} \\
\hline
\hline
Copy
 & \UseMacro{Copy-rank-long-bleu}
 & \UseMacro{Copy-rank-long-meteor}
 & \UseMacro{Copy-rank-long-rouge}
\\
ClsSubt
& \UseMacro{ClsSubt-rank-long-bleu}
& \UseMacro{ClsSubt-rank-long-meteor}
& \UseMacro{ClsSubt-rank-long-rouge}
\\
GenModel
& \UseMacro{GenModel-rank-long-bleu}
& \UseMacro{GenModel-rank-long-meteor}
& \UseMacro{GenModel-rank-long-rouge}

\\
EditModel
& \UseMacro{EditModel-rank-long-bleu}
& \UseMacro{EditModel-rank-long-meteor}
& \UseMacro{EditModel-rank-long-rouge}
\\
CopyGen
 & \UseMacro{CopyGen-rank-long-bleu}
& \UseMacro{CopyGen-rank-long-meteor}
 & \UseMacro{CopyGen-rank-long-rouge}
\\
\hline
\end{tabular}
\end{table*}


==> tables/table-models-rank-short.tex <==

%% Automatically generated by pyutil.latex 

\begin{table*}[ht]
\centering
\caption{Models number of rank 1st in short comment generation task}
\begin{tabular}{c|c|c|c|c|c|c}
\hline
\textbf{Model} & \textbf{BLEU-4} & \textbf{METEOR} &\textbf{ROUGE-l} \\
\hline
\hline
Copy
 & \UseMacro{Copy-rank-short-bleu}
 & \UseMacro{Copy-rank-short-meteor}
 & \UseMacro{Copy-rank-short-rouge}
\\
ClsSubt
& \UseMacro{ClsSubt-rank-short-bleu}
& \UseMacro{ClsSubt-rank-short-meteor}
& \UseMacro{ClsSubt-rank-short-rouge}
\\
GenModel
& \UseMacro{GenModel-rank-short-bleu}
& \UseMacro{GenModel-rank-short-meteor}
& \UseMacro{GenModel-rank-short-rouge}

\\
EditModel
& \UseMacro{EditModel-rank-short-bleu}
& \UseMacro{EditModel-rank-short-meteor}
& \UseMacro{EditModel-rank-short-rouge}
\\
CopyGen
 & \UseMacro{CopyGen-rank-short-bleu}
& \UseMacro{CopyGen-rank-short-meteor}
 & \UseMacro{CopyGen-rank-short-rouge}
\\
\hline
\end{tabular}
\end{table*}


==> tables/table-models-results.tex <==
% Manually modified on automatically generated

\begin{table*}
\small
\centering
\begin{tabular}{c|rrr|rrr}
\toprule
\multirow{2}{*}{\textbf{Model}}
  &
  \multicolumn{3}{c|}{\Short{}}
  &
  \multicolumn{3}{c}{\Long{}}
  \\
  \cline{2-7}
 & \textbf{BLEU-4} \Tstrut & \textbf{METEOR} &\textbf{ROUGE-L}
& \textbf{BLEU-4} & \textbf{METEOR} &\textbf{ROUGE-L}\\
\midrule
\UseMacro{Copy}
 & \UseMacro{Copy-short-bleu}
 & \UseMacro{Copy-short-meteor}
 & \UseMacro{Copy-short-rouge-l}
 & \UseMacro{Copy-long-bleu}
 & \UseMacro{Copy-long-meteor}
 & \UseMacro{Copy-long-rouge-l}
\\
\UseMacro{ClsSubt}
 & \UseMacro{ClsSubt-short-bleu}
 & \UseMacro{ClsSubt-short-meteor}
 & \UseMacro{ClsSubt-short-rouge-l}
 & \UseMacro{ClsSubt-long-bleu}
 & \UseMacro{ClsSubt-long-meteor}
 & \UseMacro{ClsSubt-long-rouge-l}
\\
\UseMacro{GenModel}
 & \UseMacro{GenModel-short-bleu}
 & \UseMacro{GenModel-short-meteor}
 & \UseMacro{GenModel-short-rouge-l}
 & \UseMacro{GenModel-long-bleu}
 & \UseMacro{GenModel-long-meteor}
 & \UseMacro{GenModel-long-rouge-l}
\\
\UseMacro{DeepCom}
 & \UseMacro{DeepCom-short-bleu}
 & \UseMacro{DeepCom-short-meteor}
 & \UseMacro{DeepCom-short-rouge-l}
 & \UseMacro{DeepCom-long-bleu}
 & \UseMacro{DeepCom-long-meteor}
 & \UseMacro{DeepCom-long-rouge-l}
\\
\UseMacro{EditModel}
 & \UseMacro{EditModel-feat-rerank-short-bleu}
 & \UseMacro{EditModel-feat-rerank-short-meteor}
 & \UseMacro{EditModel-feat-rerank-short-rouge-l}
 & \UseMacro{EditModel-feat-rerank-long-bleu}
 & \UseMacro{EditModel-feat-rerank-long-meteor}
 & \UseMacro{EditModel-feat-rerank-long-rouge-l}
\\
\UseMacro{CopyGen-neg-remove-overlap}
 & \textbf{\UseMacro{CopyGen-neg-remove-overlap-short-bleu}}
 & \textbf{\UseMacro{CopyGen-neg-remove-overlap-short-meteor}}
 & \textbf{\UseMacro{CopyGen-neg-remove-overlap-short-rouge-l}}
 & \textbf{\UseMacro{CopyGen-neg-remove-overlap-long-bleu}}
 & \textbf{\UseMacro{CopyGen-neg-remove-overlap-long-meteor}}
 & \textbf{\UseMacro{CopyGen-neg-remove-overlap-long-rouge-l}}
\\
\bottomrule
\end{tabular}
\caption{\TableCaptionModelsResults}
\end{table*}


==> tables/table-old-dataset-metrics.tex <==
\begin{table}
\normalsize
\centering
\begin{tabular}{l|ccc}
\hline
\textbf{} & \textbf{Train} & \textbf{Valid} & \textbf{Test} \\
\hline
 Examples&
\UseMacro{raw-train-pairs} &
\UseMacro{raw-valid-pairs} &
\UseMacro{raw-test-pairs} \\
Projects&
\UseMacro{raw-train-projects} &
\UseMacro{raw-valid-projects} &
\UseMacro{raw-test-projects} \\ 
\hline
\end{tabular}
\caption{Number of examples, projects before filtering.}\label{tab:ds-old-metrics}
\end{table}


==> tables/table-pair-example.tex <==
\begin{table*}[ht]
\centering
\caption{Hierarchy pair example}
\label{tab:table1}
\begin{tabular}{c|c|c|c}
\hline
\hline
\textbf{sup method} & \UseMacro{train-pairs} & \UseMacro{valid-pairs} & \UseMacro{test-pairs}  \\
projects & \UseMacro{train-projects} & \UseMacro{valid-projects} & \UseMacro{test-projects} \\
clean diff & \UseMacro{train-clean-diff} & \UseMacro{valid-clean-diff} & \UseMacro{test-clean-diff} \\
\hline
\end{tabular}
\end{table*}


==> tables/table-perfect-classifier.tex <==
\begin{table*}[ht]
\centering
\caption{Results given the perfect classifier}
\begin{tabular}{c|c|c|c|c|c|c}
\hline
\textbf{Model} & \textbf{Accuracy} & \textbf{BLEU-4} & \textbf{METEOR} &\textbf{SARI} &\textbf{GLEU} &\textbf{ROUGE-l} \\
\hline
\hline
editGen & 4.968 & 35.585 & 30.540 & 45.854 & 25.586 & 50.391 \\
editGen & 1.083 & 28.442 & 25.106 & 37.496 & 18.267 & 47.862 \\
\hline
\end{tabular}
\end{table*}


==> tables/table-qualitative-example-long.tex <==
\renewcommand{\arraystretch}{0.8} % Default value: 1
\begin{table*}[ht]
\centering
\begin{tabular}{l}
\toprule
{\lstinputlisting[language=java-pretty, numbers=none]{figures/Qualitative-example-long.java}}
\\
\\
\small \textbf{Gold}: clears the cache . deletes all cached files from disk .\\
\small \textbf{\Copy}: empties the cache .\\
\small \textbf{\ClassNameSubst}: empties the disk based cache .\\
\small \textbf{\SuperAgnosticGen}: removes all mappings from disk .\\
\small \textbf{\DeepCom}: deletes all cached files from disk .\\
\small \textbf{\EditModel}: clears the cache .\\ 
\small \textbf{\SuperAwareGen}: empties the cache . deletes all cached
files from disk .\\
\hline
{\lstinputlisting[language=java-pretty, numbers=none]{figures/Qualitative-example-3.java}}
\\
\\
\small \textbf{Gold}: resets this reader ' s position to the last mark ( ) location .\\
\small \textbf{\Copy}: reset the stream .\\
\small \textbf{\ClassNameSubst}: empties the disk based cache .\\
\small \textbf{\SuperAgnosticGen}: removes all of the elements from this deque .\\
\small \textbf{\DeepCom}: overrides the reader to the last marked location ( ) and reset that it can be delegated to \# sent out ( ) .\\
\small \textbf{\EditModel}: clears the stream .\\ 
\small \textbf{\SuperAwareGen}: reset the stream to the tail of this reader .\\
\bottomrule
\end{tabular}
\caption{\TableCaptionQualitativeExampleApp}
\end{table*}


==> tables/table-qualitative-example.tex <==
\renewcommand{\arraystretch}{0.9} % Default value: 1
\begin{table*}[ht]
\centering
\begin{tabular}{l}
\toprule
{\lstinputlisting[language=java-pretty, numbers=none]{figures/Qualitative-example.java}}
\\

\small \textbf{Gold}: returns asn . 1 encoded form of this info access syntax .\\
\small \textbf{\Copy}:  returns encoded form of the object .\\
\small \textbf{\ClassNameSubst}: returns encoded form of the
info access syntax .\\ 
\small \textbf{\SuperAgnosticGen}: gets the encoded value .\\
\small \textbf{\DeepCom}: returns the byte 's value of the
encoding .\\
\small \textbf{\EditModel}: returns encoding of the object .\\ 
\small \textbf{\SuperAwareGen}: returns asn 1 encoded of the info
access syntax .\\
\bottomrule
\end{tabular}
\caption{\TableCaptionQualitativeExample}
\end{table*}


==> tables/table-runtime-num-params.tex <==
\begin{table*}
\small
\centering
\begin{tabular}{c|rrr}
\toprule
\textbf{Model} & \textbf{Training Time[s]} & \textbf{Testing Time[s]} & \textbf{\#Parameters} \\
\midrule
\UseMacro{Copy} & \TableHeadNA & 6 & \TableHeadNA \\
\UseMacro{ClsSubt} & \TableHeadNA & 6 & \TableHeadNA \\
\UseMacro{GenModel} & 600 & 7,269 & 1.33M \\
\UseMacro{DeepCom} & 14,162 & 15,812 & 17.42M \\
\UseMacro{EditModel} & 1,147 & 9,384 & 2.19M \\
\UseMacro{CopyGen-neg-remove-overlap} & 919 & 8,143 & 3.33M\\
\bottomrule
\end{tabular}
\caption{Average training time, average testing time, and number of parameters of our \SuperAwareGen model and baseline models.\label{tab:runtime-num-params}}
\end{table*}


